GLYFE: Review and Benchmark of Personalized Glucose Predictive Models in Type-1 Diabetes

Due to the sensitive nature of diabetes-related data, preventing them from being shared between studies, progress in the field of glucose prediction is hard to assess. To address this issue, we present GLYFE (GLYcemia Forecasting Evaluation), a benchmark of machine-learning-based glucose-predictive models. To ensure the reproducibility of the results and the usability of the benchmark in the future, we provide extensive details about the data flow. Two datasets are used, the first comprising 10 in-silico adults from the UVA/Padova Type 1 Diabetes Metabolic Simulator (T1DMS) and the second being made of 6 real type-1 diabetic patients coming from the OhioT1DM dataset. The predictive models are personalized to the patient and evaluated on 3 different prediction horizons (30, 60, and 120 minutes) with metrics assessing their accuracy and clinical acceptability. The results of nine different models coming from the glucose-prediction literature are presented. First, they show that standard autoregressive linear models are outclassed by kernel-based non-linear ones and neural networks. In particular, the support vector regression model stands out, being at the same time one of the most accurate and clinically acceptable model. Finally, the relative performances of the models are the same for both datasets. This shows that, even though data simulated by T1DMS are not fully representative of real-world data, they can be used to assess the forecasting ability of the glucose-predictive models. Those results serve as a basis of comparison for future studies. In a field where data are hard to obtain, and where the comparison of results from different studies is often irrelevant, GLYFE gives the opportunity of gathering researchers around a standardized common environment.

==> tables/acc_tables.tex <==
\begin{table*}
\parbox{.45\linewidth}{
\caption{Mean accuracy (with standard deviation) of glucose prediction models over the T1DMS population grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_t1dms}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 22.31 \scriptsize{(3.39)} & 12.01 \scriptsize{(1.67)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{24.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 13.11 \scriptsize{(1.11)} & 7.79 \scriptsize{(0.83)} & 13.10 \scriptsize{(2.34)}\\
\textbf{ARX} & 11.52 \scriptsize{(0.84)} & 7.27 \scriptsize{(0.76)} & 15.60 \scriptsize{(1.50)}\\
\midrule
\textbf{SVR} & \textbf{9.90 \scriptsize{(0.75)}} & \textbf{6.28 \scriptsize{(0.62)}} & 19.50 \scriptsize{(2.69)}\\
\textbf{GP} & 9.97 \scriptsize{(0.69)} & 6.30 \scriptsize{(0.58)} & 19.00 \scriptsize{(2.00)}\\
\midrule
\textbf{ELM} & 11.22 \scriptsize{(1.40)} & 6.63 \scriptsize{(0.66)} & 19.50 \scriptsize{(2.69)}\\
\textbf{FFNN} & 10.34 \scriptsize{(0.74)} & 6.45 \scriptsize{(0.63)} & 19.80 \scriptsize{(2.64)}\\
\textbf{LSTM} & 10.15 \scriptsize{(0.67)} & 6.35 \scriptsize{(0.65)} & 19.00 \scriptsize{(2.57)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base} & 32.63 \scriptsize{(5.78)} & 17.75 \scriptsize{(2.97)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{54.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 24.53 \scriptsize{(3.28)} & 13.99 \scriptsize{(2.01)} & 16.30 \scriptsize{(2.49)}\\
\textbf{ARX} & 22.57 \scriptsize{(2.75)} & 13.45 \scriptsize{(1.90)} & 18.70 \scriptsize{(4.00)}\\
\midrule
\textbf{SVR} & 18.19 \scriptsize{(2.07)} & \textbf{10.72 \scriptsize{(1.43)}} & 37.80 \scriptsize{(4.19)}\\
\textbf{GP} & 18.86 \scriptsize{(2.11)} & 11.21 \scriptsize{(1.51)} & 36.20 \scriptsize{(5.23)}\\
\midrule
\textbf{ELM} & 18.82 \scriptsize{(2.40)} & 11.20 \scriptsize{(1.64)} & 38.80 \scriptsize{(3.74)}\\
\textbf{FFNN} & \textbf{17.68 \scriptsize{(1.69)}} & 10.74 \scriptsize{(1.36)} & 41.80 \scriptsize{(4.62)}\\
\textbf{LSTM} & 18.74 \scriptsize{(2.29)} & 11.36 \scriptsize{(1.60)} & 37.80 \scriptsize{(3.76)}\\

\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & 46.25 \scriptsize{(9.93)} & 26.53 \scriptsize{(5.75)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{114.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 37.55 \scriptsize{(7.45)} & 22.47 \scriptsize{(5.01)} & 18.80 \scriptsize{(6.32)}\\
\textbf{ARX} & 36.76 \scriptsize{(7.07)} & 22.26 \scriptsize{(4.80)} & 24.10 \scriptsize{(7.62)}\\
\midrule
\textbf{SVR} & 31.65 \scriptsize{(5.59)} & 17.86 \scriptsize{(3.73)} & 64.80 \scriptsize{(10.57)}\\
\textbf{GP} & 32.72 \scriptsize{(5.93)} & 19.59 \scriptsize{(4.23)} & 49.20 \scriptsize{(10.92)}\\
\midrule
\textbf{ELM} & 30.70 \scriptsize{(5.58)} & 18.32 \scriptsize{(4.12)} & 76.20 \scriptsize{(13.19)}\\
\textbf{FFNN} & \textbf{25.42 \scriptsize{(4.52)}} & \textbf{14.86 \scriptsize{(2.81)}} & 106.50 \scriptsize{(5.30)}\\
\textbf{LSTM} & 32.71 \scriptsize{(5.74)} & 20.13 \scriptsize{(4.18)} & 56.40 \scriptsize{(10.09)}\\



\bottomrule

% \bottomrule
\end{tabularx}
}
\hfill
\parbox{.45\linewidth}{
\centering
\caption{Mean accuracy (with standard deviation) of glucose prediction models over the OhioT1DM population grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_ohio}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 28.32 \scriptsize{(2.38)} & 13.51 \scriptsize{(2.72)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.32 \scriptsize{(6.62)} & 31.11 \scriptsize{(6.73)} & \textbf{23.00 \scriptsize{(10.36)}}\\
\textbf{AR} & 21.01 \scriptsize{(2.25)} & 9.61 \scriptsize{(2.24)} & 5.17 \scriptsize{(0.37)}\\
\textbf{ARX} & 20.89 \scriptsize{(2.33)} & 9.58 \scriptsize{(2.27)} & 5.00 \scriptsize{(0.00)}\\
\midrule
\textbf{SVR} & 20.55 \scriptsize{(2.49)} & \textbf{9.16 \scriptsize{(2.09)}} & 5.83 \scriptsize{(1.86)}\\
\textbf{GP} & \textbf{20.40 \scriptsize{(2.32)}} & 9.22 \scriptsize{(2.17)} & 5.83 \scriptsize{(1.86)}\\
\midrule
\textbf{ELM} & 22.30 \scriptsize{(2.02)} & 9.75 \scriptsize{(2.23)} & 5.50 \scriptsize{(2.14)}\\
\textbf{FFNN} & 20.95 \scriptsize{(2.23)} & 9.34 \scriptsize{(2.19)} & 6.17 \scriptsize{(1.86)}\\
\textbf{LSTM} & 20.57 \scriptsize{(2.15)} & 9.24 \scriptsize{(2.12)} & 6.00 \scriptsize{(1.83)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base} & 41.02 \scriptsize{(2.80)} & 20.37 \scriptsize{(3.87)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.29 \scriptsize{(6.60)} & 31.04 \scriptsize{(6.67)} & \textbf{52.50 \scriptsize{(10.52)}}\\
\textbf{AR} & 33.55 \scriptsize{(2.53)} & 16.74 \scriptsize{(3.90)} & 6.33 \scriptsize{(2.98)}\\
\textbf{ARX} & 33.43 \scriptsize{(2.53)} & 16.73 \scriptsize{(3.95)} & 5.83 \scriptsize{(1.86)}\\

\midrule
\textbf{SVR} & \textbf{32.56 \scriptsize{(2.52)}} & \textbf{15.57 \scriptsize{(3.46)}} & 8.00 \scriptsize{(3.65)}\\
\textbf{GP} & 32.59 \scriptsize{(2.45)} & 16.11 \scriptsize{(3.86)} & 7.33 \scriptsize{(3.59)}\\
\midrule
\textbf{ELM} & 33.44 \scriptsize{(2.18)} & 15.96 \scriptsize{(3.64)} & 9.17 \scriptsize{(4.78)}\\
\textbf{FFNN} & 32.92 \scriptsize{(2.61)} & 15.74 \scriptsize{(3.70)} & 9.67 \scriptsize{(4.07)}\\
\textbf{LSTM} & 32.89 \scriptsize{(2.41)} & 16.09 \scriptsize{(3.60)} & 11.33 \scriptsize{(3.86)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & 57.65 \scriptsize{(3.57)} & 30.16 \scriptsize{(4.94)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.31 \scriptsize{(6.67)} & 30.98 \scriptsize{(6.63)} & \textbf{109.67 \scriptsize{(17.29)}}\\
\textbf{AR} & 47.79 \scriptsize{(3.51)} & 25.76 \scriptsize{(5.67)} & 8.17 \scriptsize{(5.49)}\\
\textbf{ARX} & 47.76 \scriptsize{(3.40)} & 25.72 \scriptsize{(5.58)} & 8.17 \scriptsize{(4.60)}\\

\midrule
\textbf{SVR} & 47.35 \scriptsize{(2.95)} & 24.04 \scriptsize{(5.28)} & 15.17 \scriptsize{(10.35)}\\
\textbf{GP} & 47.24 \scriptsize{(3.00)} & 25.01 \scriptsize{(5.72)} & 12.67 \scriptsize{(7.27)}\\
\midrule
\textbf{ELM} & \textbf{46.50 \scriptsize{(3.15)}} & \textbf{23.88 \scriptsize{(5.25)}} & 22.83 \scriptsize{(15.85)}\\
\textbf{FFNN} & 47.09 \scriptsize{(2.86)} & 23.97 \scriptsize{(5.41)} & 26.33 \scriptsize{(15.45)}\\
\textbf{LSTM} & 47.57 \scriptsize{(2.94)} & 25.01 \scriptsize{(5.45)} & 17.17 \scriptsize{(14.06)}\\

\bottomrule
\end{tabularx}
}
\end{table*}

==> tables/h3/ohio_acc.tex <==
\begin{table}
\caption{Accuracy of glucose-predictive models, averaged over the OhioT1DM population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_ohio}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule


\textbf{Base} & 28.32 \scriptsize{(2.38)} & 13.51 \footnotesize{(2.72)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.27 \scriptsize{(6.59)} & 31.09 \scriptsize{(6.71)} & 25.50 \scriptsize{(6.87)}\\
\textbf{AR} & 20.70 \scriptsize{(2.23)} & 9.62 \scriptsize{(2.26)} & 5.17 \scriptsize{(0.37)}\\
\textbf{ARX} & & & \\
\midrule
\textbf{SVR} & 20.10 \scriptsize{(2.34)} & 9.08 \scriptsize{(2.12)} & 5.83 \scriptsize{(1.86)}\\
\textbf{GP} & 20.01 \scriptsize{(2.33)} & 9.16 \scriptsize{(2.16)} & 5.83 \scriptsize{(1.86)}\\
\midrule
\textbf{ELM} & 25.38 \scriptsize{(1.60)} & 11.56 \scriptsize{(2.43)} & 5.83 \scriptsize{(4.49)}\\
\textbf{FFNN} & 21.00 \scriptsize{(2.24)} & 9.33 \scriptsize{(2.19)} & 5.83 \scriptsize{(1.86)}\\
\textbf{LSTM} & 20.46 \scriptsize{(2.08)} & 9.24 \scriptsize{(2.10)} & 6.00 \scriptsize{(1.83)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Horizon de prédiction = 60 minutes}}}\\
\midrule

\textbf{Base} & 41.02 \scriptsize{(2.80)} & 20.37 \scriptsize{(3.87)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.27 \scriptsize{(6.58)} & 31.04 \scriptsize{(6.67)} & 56.00 \scriptsize{(6.11)}\\
\textbf{AR} & 33.20 \scriptsize{(2.69)} & 16.73 \scriptsize{(3.94)} & 6.67 \scriptsize{(3.73)}\\
\textbf{ARX} & &&\\

\midrule
\textbf{SVR} & 32.27 \scriptsize{(2.35)} & 15.38 \scriptsize{(3.43)} & 10.00 \scriptsize{(6.98)}\\
\textbf{GP} & 31.97 \scriptsize{(2.55)} & 15.92 \scriptsize{(3.80)} & 9.17 \scriptsize{(5.15)}\\
\midrule
\textbf{ELM} & 35.14 \scriptsize{(2.15)} & 16.91 \scriptsize{(3.69)} & 12.83 \scriptsize{(10.30)}\\
\textbf{FFNN} & 32.93 \scriptsize{(2.58)} & 15.83 \scriptsize{(3.97)} & 9.67 \scriptsize{(3.90)}\\
\textbf{LSTM} & 32.88 \scriptsize{(2.66)} & 16.00 \scriptsize{(3.57)} & 9.50 \scriptsize{(4.11)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Horizon de prédiction = 120 minutes}}}\\
\midrule

\textbf{Base} & 57.26 \scriptsize{(6.59)} & 31.01 \scriptsize{(6.64)} & 115.33 \scriptsize{(7.45)}\\
\midrule
\textbf{Poly} & 57.31 \scriptsize{(6.67)} & 30.98 \scriptsize{(6.63)} & \textbf{109.67 \footnotesize{(17.29)}}\\
\textbf{AR} & 47.48 \scriptsize{(3.75)} & 25.69 \scriptsize{(5.79)} & 9.83 \scriptsize{(6.72)}\\
\textbf{ARX} & &&\\

\midrule
\textbf{SVR} & 46.96 \scriptsize{(2.67)} & 23.45 \scriptsize{(4.96)} & 25.00 \scriptsize{(23.09)}\\
\textbf{GP} & 46.24 \scriptsize{(2.86)} & 24.65 \scriptsize{(5.69)} & 20.33 \scriptsize{(15.25)}\\
\midrule
\textbf{ELM} & 46.64 \scriptsize{(3.38)} & 24.28 \scriptsize{(5.16)} & 31.83 \scriptsize{(25.02)}\\
\textbf{FFNN} & 46.86 \scriptsize{(2.83)} & 23.82 \scriptsize{(5.39)} & 33.17 \scriptsize{(23.34)}\\
\textbf{LSTM} & 47.56 \scriptsize{(3.05)} & 24.69 \scriptsize{(5.34)} & 21.33 \scriptsize{(15.22)}\\

\bottomrule
\end{tabularx}

\end{table}


==> tables/h3/t1dms_acc.tex <==
\begin{table}
\caption{Accuracy of glucose-predictive models, averaged over the T1DMS population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_t1dms}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 22.31 \scriptsize{(3.39)} & 12.01 \scriptsize{(1.67)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{24.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 13.08 \scriptsize{(1.13)} & 7.77 \scriptsize{(0.83)} & 13.30 \scriptsize{(2.15)}\\
\textbf{ARX} & &&\\
\midrule
\textbf{SVR} & 9.05 \scriptsize{(0.51)} & 5.90 \scriptsize{(0.60)} & 22.80 \scriptsize{(2.36)}\\
\textbf{GP} & 9.00 \scriptsize{(0.54)} & 5.88 \scriptsize{(0.56)} & 22.50 \scriptsize{(2.50)}\\
\midrule
\textbf{ELM} & 13.39 \scriptsize{(2.53)} & 7.33 \scriptsize{(0.84)} & 24.50 \scriptsize{(1.20)}\\
\textbf{FFNN} & 10.37 \scriptsize{(0.73)} & 6.46 \scriptsize{(0.61)} & 19.60 \scriptsize{(2.76)}\\
\textbf{LSTM} & 10.14 \scriptsize{(0.78)} & 6.35 \scriptsize{(0.64)} & 18.60 \scriptsize{(2.11)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Horizon de prédiction = 60 minutes}}}\\
\midrule

\textbf{Base} & 32.63 \scriptsize{(5.78)} & 17.75 \scriptsize{(2.97)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{54.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 24.44 \scriptsize{(3.32)} & 13.94 \scriptsize{(1.98)} & 16.50 \scriptsize{(2.29)}\\
\textbf{ARX} & &&\\
\midrule
\textbf{SVR} & 16.07 \scriptsize{(1.53)} & 9.52 \scriptsize{(1.22)} & 44.00 \scriptsize{(2.19)}\\
\textbf{GP} & 16.19 \scriptsize{(1.56)} & 9.84 \scriptsize{(1.25)} & 42.30 \scriptsize{(2.37)}\\
\midrule
\textbf{ELM} & 18.40 \scriptsize{(2.89)} & 10.52 \scriptsize{(1.51)} & 48.00 \scriptsize{(2.14)}\\
\textbf{FFNN} & 17.84 \scriptsize{(1.65)} & 10.82 \scriptsize{(1.29)} & 43.70 \scriptsize{(4.15)}\\
\textbf{LSTM} & 18.66 \scriptsize{(1.95)} & 11.34 \scriptsize{(1.63)} & 37.70 \scriptsize{(4.10)}\\

\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Horizon de prédiction = 120 minutes}}}\\
\midrule

\textbf{Base} & 46.25 \scriptsize{(9.93)} & 26.53 \scriptsize{(5.75)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{114.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 37.42 \scriptsize{(7.43)} & 22.38 \scriptsize{(4.87)} & 20.10 \scriptsize{(5.94)}\\
\textbf{ARX} & &&\\
\midrule
\textbf{SVR} & 26.55 \scriptsize{(4.96)} & 14.26 \scriptsize{(2.56)} & 94.00 \scriptsize{(13.21)}\\
\textbf{GP} & 27.27 \scriptsize{(4.74)} & 15.85 \scriptsize{(2.81)} & 73.00 \scriptsize{(10.78)}\\
\midrule
\textbf{ELM} & 26.75 \scriptsize{(4.71)} & 14.81 \scriptsize{(2.59)} & 108.70 \scriptsize{(5.90)}\\
\textbf{FFNN} & 25.48 \scriptsize{(4.54)} & 14.71 \scriptsize{(2.90)} & 104.70 \scriptsize{(4.71)}\\
\textbf{LSTM} & 32.78 \scriptsize{(5.81)} & 20.21 \scriptsize{(4.14)} & 56.00 \scriptsize{(9.27)}\\



\bottomrule

% \bottomrule
\end{tabularx}

\end{table}


==> tables/ohio_acc.tex <==
\begin{table}
\caption{Accuracy of glucose-predictive models, averaged over the OhioT1DM population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_ohio}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 28.32 \scriptsize{(2.38)} & 13.51 \scriptsize{(2.72)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.32 \scriptsize{(6.62)} & 31.11 \scriptsize{(6.73)} & \textbf{23.00 \scriptsize{(10.36)}}\\
\textbf{AR} & 21.01 \scriptsize{(2.25)} & 9.61 \scriptsize{(2.24)} & 5.17 \scriptsize{(0.37)}\\
\textbf{ARX} & 20.89 \scriptsize{(2.33)} & 9.58 \scriptsize{(2.27)} & 5.00 \scriptsize{(0.00)}\\
\midrule
\textbf{SVR} & 20.55 \scriptsize{(2.49)} & \textbf{9.16 \scriptsize{(2.09)}} & 5.83 \scriptsize{(1.86)}\\
\textbf{GP} & \textbf{20.40 \scriptsize{(2.32)}} & 9.22 \scriptsize{(2.17)} & 5.83 \scriptsize{(1.86)}\\
\midrule
\textbf{ELM} & 22.30 \scriptsize{(2.02)} & 9.75 \scriptsize{(2.23)} & 5.50 \scriptsize{(2.14)}\\
\textbf{FFNN} & 20.95 \scriptsize{(2.23)} & 9.34 \scriptsize{(2.19)} & 6.17 \scriptsize{(1.86)}\\
\textbf{LSTM} & 20.57 \scriptsize{(2.15)} & 9.24 \scriptsize{(2.12)} & 6.00 \scriptsize{(1.83)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base} & 41.02 \scriptsize{(2.80)} & 20.37 \scriptsize{(3.87)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.29 \scriptsize{(6.60)} & 31.04 \scriptsize{(6.67)} & \textbf{52.50 \scriptsize{(10.52)}}\\
\textbf{AR} & 33.55 \scriptsize{(2.53)} & 16.74 \scriptsize{(3.90)} & 6.33 \scriptsize{(2.98)}\\
\textbf{ARX} & 33.43 \scriptsize{(2.53)} & 16.73 \scriptsize{(3.95)} & 5.83 \scriptsize{(1.86)}\\

\midrule
\textbf{SVR} & \textbf{32.56 \scriptsize{(2.52)}} & \textbf{15.57 \scriptsize{(3.46)}} & 8.00 \scriptsize{(3.65)}\\
\textbf{GP} & 32.59 \scriptsize{(2.45)} & 16.11 \scriptsize{(3.86)} & 7.33 \scriptsize{(3.59)}\\
\midrule
\textbf{ELM} & 33.44 \scriptsize{(2.18)} & 15.96 \scriptsize{(3.64)} & 9.17 \scriptsize{(4.78)}\\
\textbf{FFNN} & 32.92 \scriptsize{(2.61)} & 15.74 \scriptsize{(3.70)} & 9.67 \scriptsize{(4.07)}\\
\textbf{LSTM} & 32.89 \scriptsize{(2.41)} & 16.09 \scriptsize{(3.60)} & 11.33 \scriptsize{(3.86)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & 57.65 \scriptsize{(3.57)} & 30.16 \scriptsize{(4.94)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 57.31 \scriptsize{(6.67)} & 30.98 \scriptsize{(6.63)} & \textbf{109.67 \scriptsize{(17.29)}}\\
\textbf{AR} & 47.79 \scriptsize{(3.51)} & 25.76 \scriptsize{(5.67)} & 8.17 \scriptsize{(5.49)}\\
\textbf{ARX} & 47.76 \scriptsize{(3.40)} & 25.72 \scriptsize{(5.58)} & 8.17 \scriptsize{(4.60)}\\

\midrule
\textbf{SVR} & 47.35 \scriptsize{(2.95)} & 24.04 \scriptsize{(5.28)} & 15.17 \scriptsize{(10.35)}\\
\textbf{GP} & 47.24 \scriptsize{(3.00)} & 25.01 \scriptsize{(5.72)} & 12.67 \scriptsize{(7.27)}\\
\midrule
\textbf{ELM} & \textbf{46.50 \scriptsize{(3.15)}} & \textbf{23.88 \scriptsize{(5.25)}} & 22.83 \scriptsize{(15.85)}\\
\textbf{FFNN} & 47.09 \scriptsize{(2.86)} & 23.97 \scriptsize{(5.41)} & 26.33 \scriptsize{(15.45)}\\
\textbf{LSTM} & 47.57 \scriptsize{(2.94)} & 25.01 \scriptsize{(5.45)} & 17.17 \scriptsize{(14.06)}\\

\bottomrule
\end{tabularx}

\end{table}


==> tables/ohio_cg_ega.tex <==
\begin{table*}
\caption{Clinical acceptability of glucose-predictive models, averaged over the OhioT1DM population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:cgega_ohio}
\begin{tabularx}{\textwidth}{@{}l||*{3}{C}|*{3}{C}|*{3}{C}@{}}
\toprule

\multirow{3}{*}{\textbf{Models}} &    \multicolumn{9}{c}{\textbf{CG-EGA}} \\

& \multicolumn{3}{c|}{\textit{Hypoglycemia}} & \multicolumn{3}{c|}{\textit{Euglycemia}} & \multicolumn{3}{c}{\textit{Hyperglycemia}} \\ 

& AP & BE & EP & AP & BE & EP & AP & BE & EP \\


\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 39.24 \scriptsize{(16.93)} & 2.82 \scriptsize{(4.17)} & 57.94 \scriptsize{(18.85)} & 90.25 \scriptsize{(3.40)} & 7.11 \scriptsize{(2.44)} & 2.64 \scriptsize{(1.15)} & \textbf{84.40 \scriptsize{(3.88)}} & 11.44 \scriptsize{(2.59)} & \textbf{4.16 \scriptsize{(1.83)}}\\
\midrule
\textbf{Poly} & 0.00 \scriptsize{(0.00)} & \textbf{0.00 \scriptsize{(0.00)}} & 100.00 \scriptsize{(0.00)} & \textbf{94.54 \scriptsize{(1.74)}} & \textbf{5.20 \scriptsize{(1.84)}} & \textbf{0.27 \scriptsize{(0.55)}} & 75.71 \scriptsize{(6.30)} & \textbf{7.00 \scriptsize{(2.82)}} & 17.29 \scriptsize{(5.72)}\\
\textbf{AR} & 39.91 \scriptsize{(21.56)} & 4.74 \scriptsize{(3.61)} & 55.34 \scriptsize{(23.01)} & 84.69 \scriptsize{(5.31)} & 12.06 \scriptsize{(4.04)} & 3.25 \scriptsize{(1.40)} & 78.41 \scriptsize{(2.91)} & 16.61 \scriptsize{(3.01)} & 4.98 \scriptsize{(1.77)}\\
\textbf{ARX} & 40.19 \scriptsize{(22.60)} & 4.94 \scriptsize{(3.32)} & 54.87 \scriptsize{(23.79)} & 84.54 \scriptsize{(5.43)} & 12.17 \scriptsize{(4.23)} & 3.29 \scriptsize{(1.39)} & 78.24 \scriptsize{(3.12)} & 16.71 \scriptsize{(3.25)} & 5.05 \scriptsize{(1.87)}\\

\midrule
\textbf{SVR} & 46.13 \scriptsize{(26.62)} & 4.83 \scriptsize{(4.57)} & 49.03 \scriptsize{(26.94)} & 85.24 \scriptsize{(5.31)} & 11.65 \scriptsize{(4.09)} & 3.11 \scriptsize{(1.39)} & 78.67 \scriptsize{(4.38)} & 16.37 \scriptsize{(3.88)} & 4.95 \scriptsize{(2.30)}\\
\textbf{GP} & 46.76 \scriptsize{(26.14)} & 5.38 \scriptsize{(4.07)} & 47.87 \scriptsize{(27.36)} & 84.21 \scriptsize{(5.22)} & 12.57 \scriptsize{(4.07)} & 3.22 \scriptsize{(1.37)} & 77.78 \scriptsize{(3.61)} & 17.16 \scriptsize{(3.01)} & 5.06 \scriptsize{(1.80)}\\
\midrule
\textbf{ELM} & \textbf{56.92 \scriptsize{(22.61)}} & 4.13 \scriptsize{(3.87)} & \textbf{38.95 \scriptsize{(20.28)}} & 83.57 \scriptsize{(4.76)} & 13.07 \scriptsize{(3.80)} & 3.36 \scriptsize{(1.28)} & 76.32 \scriptsize{(4.48)} & 18.27 \scriptsize{(3.35)} & 5.41 \scriptsize{(2.46)}\\
\textbf{FFNN} & 47.77 \scriptsize{(25.48)} & 2.99 \scriptsize{(2.79)} & 49.24 \scriptsize{(25.81)} & 82.63 \scriptsize{(5.30)} & 13.68 \scriptsize{(4.03)} & 3.70 \scriptsize{(1.40)} & 74.85 \scriptsize{(3.92)} & 19.42 \scriptsize{(3.41)} & 5.73 \scriptsize{(2.20)}\\
\textbf{LSTM} & 39.57 \scriptsize{(23.35)} & 3.22 \scriptsize{(2.88)} & 57.21 \scriptsize{(23.75)} & 83.84 \scriptsize{(5.80)} & 12.62 \scriptsize{(4.43)} & 3.54 \scriptsize{(1.52)} & 76.86 \scriptsize{(4.30)} & 17.74 \scriptsize{(3.09)} & 5.40 \scriptsize{(2.44)}\\




\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base} & \textbf{20.00 \scriptsize{(15.92)}} & 2.86 \scriptsize{(3.12)} & \textbf{77.14 \scriptsize{(15.32)}} & 88.27 \scriptsize{(4.23)} & 8.22 \scriptsize{(2.57)} & 3.51 \scriptsize{(1.72)} & \textbf{81.77 \scriptsize{(4.65)}} & 12.06 \scriptsize{(2.43)} & \textbf{6.17 \scriptsize{(2.33)}}\\
\midrule
\textbf{Poly} & 0.00 \scriptsize{(0.00)} & \textbf{0.00 \scriptsize{(0.00)}} & 100.00 \scriptsize{(0.00)} & \textbf{94.77 \scriptsize{(1.85)}} & \textbf{5.13 \scriptsize{(1.90)}} & \textbf{0.10 \scriptsize{(0.18)}} & 75.87 \scriptsize{(6.23)} & \textbf{6.99 \scriptsize{(2.86)}} & 17.14 \scriptsize{(5.74)}\\
\textbf{AR} & 7.32 \scriptsize{(7.10)} & 2.02 \scriptsize{(2.26)} & 90.66 \scriptsize{(8.41)} & 82.47 \scriptsize{(4.74)} & 13.34 \scriptsize{(3.61)} & 4.19 \scriptsize{(1.28)} & 74.08 \scriptsize{(4.52)} & 18.11 \scriptsize{(2.78)} & 7.81 \scriptsize{(3.34)}\\
\textbf{ARX} & 7.67 \scriptsize{(7.42)} & 1.97 \scriptsize{(2.30)} & 90.36 \scriptsize{(8.90)} & 82.12 \scriptsize{(4.92)} & 13.69 \scriptsize{(3.81)} & 4.19 \scriptsize{(1.28)} & 73.78 \scriptsize{(4.64)} & 18.54 \scriptsize{(3.10)} & 7.67 \scriptsize{(3.09)}\\

\midrule
\textbf{SVR} & 14.77 \scriptsize{(11.92)} & 2.59 \scriptsize{(2.02)} & 82.64 \scriptsize{(13.14)} & 81.96 \scriptsize{(5.48)} & 13.87 \scriptsize{(4.11)} & 4.17 \scriptsize{(1.48)} & 73.94 \scriptsize{(5.85)} & 18.70 \scriptsize{(3.50)} & 7.36 \scriptsize{(3.09)}\\
\textbf{GP} & 11.44 \scriptsize{(8.74)} & 2.23 \scriptsize{(2.03)} & 86.33 \scriptsize{(10.26)} & 81.59 \scriptsize{(5.15)} & 14.19 \scriptsize{(3.89)} & 4.22 \scriptsize{(1.43)} & 73.81 \scriptsize{(5.20)} & 18.80 \scriptsize{(2.98)} & 7.39 \scriptsize{(2.90)}\\
\midrule
\textbf{ELM} & 12.02 \scriptsize{(13.64)} & 1.27 \scriptsize{(1.57)} & 86.71 \scriptsize{(14.91)} & 81.75 \scriptsize{(4.42)} & 14.37 \scriptsize{(3.39)} & 3.88 \scriptsize{(1.26)} & 74.59 \scriptsize{(5.71)} & 17.95 \scriptsize{(3.15)} & 7.46 \scriptsize{(3.30)}\\
\textbf{FFNN} & 10.77 \scriptsize{(11.41)} & 0.89 \scriptsize{(1.12)} & 88.34 \scriptsize{(12.43)} & 78.97 \scriptsize{(5.54)} & 16.57 \scriptsize{(4.22)} & 4.46 \scriptsize{(1.52)} & 69.35 \scriptsize{(6.19)} & 22.30 \scriptsize{(3.59)} & 8.35 \scriptsize{(3.42)}\\
\textbf{LSTM} & 3.49 \scriptsize{(4.42)} & 1.27 \scriptsize{(1.01)} & 95.24 \scriptsize{(4.99)} & 82.07 \scriptsize{(4.99)} & 13.88 \scriptsize{(3.64)} & 4.05 \scriptsize{(1.49)} & 72.06 \scriptsize{(6.09)} & 19.83 \scriptsize{(2.75)} & 8.11 \scriptsize{(3.67)}\\



\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & \textbf{7.76 \scriptsize{(6.78)}} & 0.91 \scriptsize{(1.02)} & 91.33 \scriptsize{(6.98)} & 85.06 \scriptsize{(3.88)} & 9.09 \scriptsize{(2.92)} & 5.85 \scriptsize{(1.08)} & \textbf{78.58 \scriptsize{(5.01)}} & 12.07 \scriptsize{(2.41)} & \textbf{9.36 \scriptsize{(3.25)}}\\
\midrule
\textbf{Poly} & 0.00 \scriptsize{(0.00)} & \textbf{0.00 \scriptsize{(0.00)}} & 100.00 \scriptsize{(0.00)} & 94.80 \scriptsize{(1.83)} & \textbf{5.10 \scriptsize{(1.87)}} & 0.10 \scriptsize{(0.15)} & 75.88 \scriptsize{(6.16)} & 7.00 \scriptsize{(2.89)} & 17.12 \scriptsize{(5.63)}\\
\textbf{AR} & 0.00 \scriptsize{(0.00)} & \textbf{0.00 \scriptsize{(0.00)}} & 100.00 \scriptsize{(0.00)} & \textbf{94.82 \scriptsize{(1.81)}} & 5.18 \scriptsize{(1.81)} & \textbf{0.00 \scriptsize{(0.00)}} & 75.75 \scriptsize{(11.38)} & \textbf{6.97 \scriptsize{(2.29)}} & 17.27 \scriptsize{(9.71)}\\
\textbf{ARX} & 0.00 \scriptsize{(0.00)} & \textbf{0.00 \scriptsize{(0.00)}} & 100.00 \scriptsize{(0.00)} & 84.90 \scriptsize{(3.61)} & 11.63 \scriptsize{(2.81)} & 3.47 \scriptsize{(1.07)} & 74.56 \scriptsize{(6.02)} & 14.20 \scriptsize{(2.18)} & 11.24 \scriptsize{(4.71)}\\
\midrule
\textbf{SVR} & 6.61 \scriptsize{(6.91)} & 4.25 \scriptsize{(7.07)} & \textbf{89.14 \scriptsize{(13.21)}} & 83.83 \scriptsize{(3.11)} & 12.67 \scriptsize{(2.40)} & 3.51 \scriptsize{(1.19)} & 74.21 \scriptsize{(4.95)} & 14.59 \scriptsize{(2.57)} & 11.20 \scriptsize{(4.38)}\\
\textbf{GP} & 1.69 \scriptsize{(1.98)} & 0.31 \scriptsize{(0.58)} & 98.00 \scriptsize{(2.47)} & 83.34 \scriptsize{(3.64)} & 12.87 \scriptsize{(2.75)} & 3.79 \scriptsize{(1.19)} & 73.44 \scriptsize{(5.84)} & 15.39 \scriptsize{(2.35)} & 11.17 \scriptsize{(4.25)}\\
\midrule
\textbf{ELM} & 1.95 \scriptsize{(3.68)} & 0.40 \scriptsize{(0.57)} & 97.65 \scriptsize{(4.16)} & 82.79 \scriptsize{(2.18)} & 13.52 \scriptsize{(1.07)} & 3.69 \scriptsize{(1.27)} & 74.82 \scriptsize{(4.73)} & 14.38 \scriptsize{(1.83)} & 10.79 \scriptsize{(4.60)}\\
\textbf{FFNN} & 2.92 \scriptsize{(2.88)} & 2.55 \scriptsize{(4.36)} & 94.54 \scriptsize{(6.75)} & 77.63 \scriptsize{(3.38)} & 18.15 \scriptsize{(2.52)} & 4.22 \scriptsize{(1.12)} & 69.16 \scriptsize{(5.40)} & 19.45 \scriptsize{(2.39)} & 11.39 \scriptsize{(4.52)}\\
\textbf{LSTM} & 1.10 \scriptsize{(1.99)} & 0.61 \scriptsize{(1.36)} & 98.29 \scriptsize{(3.33)} & 83.88 \scriptsize{(3.51)} & 12.70 \scriptsize{(2.66)} & 3.42 \scriptsize{(1.05)} & 74.40 \scriptsize{(6.50)} & 15.04 \scriptsize{(2.70)} & 10.56 \scriptsize{(4.61)}\\



\bottomrule

\end{tabularx}


\begin{flushright}
AP: Accurate Prediction; BE: Benign Error; EP: Erroneous Prediction
\end{flushright}


\end{table*}


==> tables/t1dms_acc.tex <==
\begin{table}
\caption{Accuracy of glucose-predictive models, averaged over the T1DMS population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:acc_t1dms}
\begin{tabularx}{\linewidth}{l||C|C|C}
\toprule

\textbf{Models} &  \textbf{RMSE} &\textbf{MAPE} & \textbf{TG}   \\



\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 22.31 \scriptsize{(3.39)} & 12.01 \scriptsize{(1.67)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{24.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 13.11 \scriptsize{(1.11)} & 7.79 \scriptsize{(0.83)} & 13.10 \scriptsize{(2.34)}\\
\textbf{ARX} & 11.52 \scriptsize{(0.84)} & 7.27 \scriptsize{(0.76)} & 15.60 \scriptsize{(1.50)}\\
\midrule
\textbf{SVR} & \textbf{9.90 \scriptsize{(0.75)}} & \textbf{6.28 \scriptsize{(0.62)}} & 19.50 \scriptsize{(2.69)}\\
\textbf{GP} & 9.97 \scriptsize{(0.69)} & 6.30 \scriptsize{(0.58)} & 19.00 \scriptsize{(2.00)}\\
\midrule
\textbf{ELM} & 11.22 \scriptsize{(1.40)} & 6.63 \scriptsize{(0.66)} & 19.50 \scriptsize{(2.69)}\\
\textbf{FFNN} & 10.34 \scriptsize{(0.74)} & 6.45 \scriptsize{(0.63)} & 19.80 \scriptsize{(2.64)}\\
\textbf{LSTM} & 10.15 \scriptsize{(0.67)} & 6.35 \scriptsize{(0.65)} & 19.00 \scriptsize{(2.57)}\\


\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base} & 32.63 \scriptsize{(5.78)} & 17.75 \scriptsize{(2.97)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{54.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 24.53 \scriptsize{(3.28)} & 13.99 \scriptsize{(2.01)} & 16.30 \scriptsize{(2.49)}\\
\textbf{ARX} & 22.57 \scriptsize{(2.75)} & 13.45 \scriptsize{(1.90)} & 18.70 \scriptsize{(4.00)}\\
\midrule
\textbf{SVR} & 18.19 \scriptsize{(2.07)} & \textbf{10.72 \scriptsize{(1.43)}} & 37.80 \scriptsize{(4.19)}\\
\textbf{GP} & 18.86 \scriptsize{(2.11)} & 11.21 \scriptsize{(1.51)} & 36.20 \scriptsize{(5.23)}\\
\midrule
\textbf{ELM} & 18.82 \scriptsize{(2.40)} & 11.20 \scriptsize{(1.64)} & 38.80 \scriptsize{(3.74)}\\
\textbf{FFNN} & \textbf{17.68 \scriptsize{(1.69)}} & 10.74 \scriptsize{(1.36)} & 41.80 \scriptsize{(4.62)}\\
\textbf{LSTM} & 18.74 \scriptsize{(2.29)} & 11.36 \scriptsize{(1.60)} & 37.80 \scriptsize{(3.76)}\\

\midrule
\midrule
\multicolumn{4}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & 46.25 \scriptsize{(9.93)} & 26.53 \scriptsize{(5.75)} & 0.00 \scriptsize{(0.00)}\\
\midrule
\textbf{Poly} & 42.94 \scriptsize{(15.40)} & 25.63 \scriptsize{(10.55)} & \textbf{114.10 \scriptsize{(2.70)}}\\
\textbf{AR} & 37.55 \scriptsize{(7.45)} & 22.47 \scriptsize{(5.01)} & 18.80 \scriptsize{(6.32)}\\
\textbf{ARX} & 36.76 \scriptsize{(7.07)} & 22.26 \scriptsize{(4.80)} & 24.10 \scriptsize{(7.62)}\\
\midrule
\textbf{SVR} & 31.65 \scriptsize{(5.59)} & 17.86 \scriptsize{(3.73)} & 64.80 \scriptsize{(10.57)}\\
\textbf{GP} & 32.72 \scriptsize{(5.93)} & 19.59 \scriptsize{(4.23)} & 49.20 \scriptsize{(10.92)}\\
\midrule
\textbf{ELM} & 30.70 \scriptsize{(5.58)} & 18.32 \scriptsize{(4.12)} & 76.20 \scriptsize{(13.19)}\\
\textbf{FFNN} & \textbf{25.42 \scriptsize{(4.52)}} & \textbf{14.86 \scriptsize{(2.81)}} & 106.50 \scriptsize{(5.30)}\\
\textbf{LSTM} & 32.71 \scriptsize{(5.74)} & 20.13 \scriptsize{(4.18)} & 56.40 \scriptsize{(10.09)}\\



\bottomrule

% \bottomrule
\end{tabularx}

\end{table}


==> tables/t1dms_cg_ega.tex <==
\begin{table*}
\caption{Clinical acceptability of glucose-predictive models, averaged over the OhioT1DM population (with standard deivation), and grouped by prediction horizon (30, 60, and 120 minutes).}
\label{table:cgega_t1dms}
\begin{tabularx}{\textwidth}{@{}l||*{3}{C}|*{3}{C}|*{3}{C}@{}}
\toprule

\multirow{3}{*}{\textbf{Models}} &    \multicolumn{9}{c}{\textbf{CG-EGA}} \\

& \multicolumn{3}{c|}{\textit{Hypoglycemia}} & \multicolumn{3}{c|}{\textit{Euglycemia}} & \multicolumn{3}{c}{\textit{Hyperglycemia}} \\ 

& AP & BE & EP & AP & BE & EP & AP & BE & EP \\


\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 30 minutes}}}\\
\midrule

\textbf{Base} & 73.52 \scriptsize{(14.09)} & 2.18 \scriptsize{(3.86)} & 24.30 \scriptsize{(11.79)} & 95.98 \scriptsize{(1.05)} & 3.47 \scriptsize{(0.85)} & 0.56 \scriptsize{(0.31)} & 85.94 \scriptsize{(9.07)} & 10.88 \scriptsize{(6.87)} & 3.18 \scriptsize{(2.38)}\\
\midrule
\textbf{Poly} & 0.11 \scriptsize{(0.33)} & \textbf{0.00 \scriptsize{(0.00)}} & 99.89 \scriptsize{(0.33)} & \textbf{99.27 \scriptsize{(0.33)}} & \textbf{0.68 \scriptsize{(0.31)}} & \textbf{0.05 \scriptsize{(0.06)}} & 79.88 \scriptsize{(7.80)} & \textbf{2.11 \scriptsize{(1.35)}} & 18.02 \scriptsize{(7.57)}\\
\textbf{AR} & 64.10 \scriptsize{(10.09)} & 14.22 \scriptsize{(7.81)} & 21.69 \scriptsize{(10.82)} & 79.77 \scriptsize{(3.24)} & 18.02 \scriptsize{(2.67)} & 2.21 \scriptsize{(0.65)} & 79.42 \scriptsize{(4.52)} & 18.18 \scriptsize{(3.72)} & 2.40 \scriptsize{(0.97)}\\
\textbf{ARX} & 72.63 \scriptsize{(8.42)} & 11.49 \scriptsize{(5.43)} & 15.88 \scriptsize{(6.69)} & 83.03 \scriptsize{(2.49)} & 15.20 \scriptsize{(2.11)} & 1.77 \scriptsize{(0.54)} & 82.13 \scriptsize{(4.14)} & 15.66 \scriptsize{(3.32)} & 2.21 \scriptsize{(1.11)}\\
\midrule
\textbf{SVR} & 84.02 \scriptsize{(10.95)} & 4.34 \scriptsize{(4.93)} & 11.64 \scriptsize{(6.43)} & 94.45 \scriptsize{(1.16)} & 4.68 \scriptsize{(0.89)} & 0.87 \scriptsize{(0.33)} & 91.29 \scriptsize{(2.29)} & 7.11 \scriptsize{(1.69)} & 1.60 \scriptsize{(0.80)}\\
\textbf{GP} & 83.71 \scriptsize{(9.77)} & 7.34 \scriptsize{(4.44)} & \textbf{8.94 \scriptsize{(7.84)}} & 91.39 \scriptsize{(1.82)} & 7.48 \scriptsize{(1.59)} & 1.13 \scriptsize{(0.36)} & 90.49 \scriptsize{(1.54)} & 8.04 \scriptsize{(1.06)} & 1.47 \scriptsize{(0.67)}\\
\midrule
\textbf{ELM} & 84.89 \scriptsize{(7.02)} & 2.80 \scriptsize{(3.34)} & 12.31 \scriptsize{(4.49)} & 95.24 \scriptsize{(1.04)} & 4.03 \scriptsize{(0.79)} & 0.74 \scriptsize{(0.33)} & \textbf{92.08 \scriptsize{(2.28)}} & 6.49 \scriptsize{(1.95)} & 1.43 \scriptsize{(0.70)}\\
\textbf{FFNN} & 86.18 \scriptsize{(5.76)} & 3.51 \scriptsize{(3.12)} & 10.31 \scriptsize{(3.40)} & 95.21 \scriptsize{(0.72)} & 4.01 \scriptsize{(0.47)} & 0.78 \scriptsize{(0.32)} & 91.72 \scriptsize{(2.24)} & 6.85 \scriptsize{(1.91)} & \textbf{1.43 \scriptsize{(0.58)}}\\
\textbf{LSTM} & \textbf{86.33 \scriptsize{(9.23)}} & 3.93 \scriptsize{(4.15)} & 9.74 \scriptsize{(5.41)} & 93.82 \scriptsize{(1.01)} & 5.27 \scriptsize{(0.82)} & 0.91 \scriptsize{(0.33)} & 91.58 \scriptsize{(2.23)} & 6.98 \scriptsize{(1.89)} & 1.45 \scriptsize{(0.66)}\\

\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 60 minutes}}}\\
\midrule

\textbf{Base}& 39.98 \scriptsize{(22.15)} & 1.50 \scriptsize{(2.52)} & 58.51 \scriptsize{(21.89)} & 95.55 \scriptsize{(1.53)} & 3.60 \scriptsize{(1.26)} & 0.85 \scriptsize{(0.41)} & 81.41 \scriptsize{(7.75)} & 11.30 \scriptsize{(5.00)} & 7.29 \scriptsize{(3.54)}\\
\midrule
\textbf{Poly} & 0.11 \scriptsize{(0.33)} & \textbf{\textbf{0.00 \scriptsize{(0.00)}}} & 99.89 \scriptsize{(0.33)} & \textbf{99.27 \scriptsize{(0.33)}} & \textbf{0.68 \scriptsize{(0.31)}} & \textbf{0.05 \scriptsize{(0.06)}} & 79.88 \scriptsize{(7.80)} & \textbf{2.11 \scriptsize{(1.35)}} & 18.02 \scriptsize{(7.57)}\\
\textbf{AR} & 21.24 \scriptsize{(15.53)} & 8.78 \scriptsize{(5.69)} & 69.98 \scriptsize{(20.67)} & 77.06 \scriptsize{(6.08)} & 20.36 \scriptsize{(5.27)} & 2.58 \scriptsize{(0.88)} & 69.64 \scriptsize{(6.90)} & 23.43 \scriptsize{(4.33)} & 6.93 \scriptsize{(2.84)}\\
\textbf{ARX} & 23.15 \scriptsize{(16.21)} & 9.48 \scriptsize{(5.73)} & 67.36 \scriptsize{(20.76)} & 77.16 \scriptsize{(5.51)} & 20.31 \scriptsize{(4.67)} & 2.53 \scriptsize{(0.89)} & 71.56 \scriptsize{(6.15)} & 22.86 \scriptsize{(4.27)} & 5.58 \scriptsize{(1.99)}\\
\midrule
\textbf{SVR} & 42.98 \scriptsize{(20.97)} & 2.80 \scriptsize{(2.56)} & 54.22 \scriptsize{(21.46)} & 92.92 \scriptsize{(2.08)} & 6.20 \scriptsize{(1.68)} & 0.88 \scriptsize{(0.42)} & 84.58 \scriptsize{(3.97)} & 12.99 \scriptsize{(3.47)} & 2.43 \scriptsize{(0.89)}\\
\textbf{GP} & 36.44 \scriptsize{(21.75)} & 3.99 \scriptsize{(3.18)} & 59.57 \scriptsize{(24.45)} & 88.88 \scriptsize{(4.01)} & 9.58 \scriptsize{(3.40)} & 1.54 \scriptsize{(0.66)} & 81.94 \scriptsize{(4.80)} & 15.12 \scriptsize{(4.40)} & 2.94 \scriptsize{(0.99)}\\
\midrule
\textbf{ELM} & 41.87 \scriptsize{(20.04)} & 3.39 \scriptsize{(2.93)} & 54.75 \scriptsize{(20.85)} & 92.80 \scriptsize{(2.60)} & 6.33 \scriptsize{(2.14)} & 0.87 \scriptsize{(0.50)} & \textbf{85.72 \scriptsize{(4.18)}} & 12.13 \scriptsize{(3.40)} & \textbf{2.15 \scriptsize{(1.16)}}\\
\textbf{FFNN} & \textbf{46.62 \scriptsize{(19.77)}} & 3.50 \scriptsize{(2.59)} & \textbf{49.88 \scriptsize{(20.37)}} & 91.12 \scriptsize{(2.27)} & 7.97 \scriptsize{(1.96)} & 0.91 \scriptsize{(0.39)} & 80.67 \scriptsize{(4.17)} & 16.72 \scriptsize{(3.70)} & 2.62 \scriptsize{(1.14)}\\
\textbf{LSTM} & 42.70 \scriptsize{(19.12)} & 3.71 \scriptsize{(3.45)} & 53.59 \scriptsize{(20.07)} & 92.21 \scriptsize{(2.94)} & 6.87 \scriptsize{(2.48)} & 0.92 \scriptsize{(0.49)} & 85.19 \scriptsize{(3.40)} & 12.30 \scriptsize{(3.06)} & 2.52 \scriptsize{(0.74)}\\

\midrule
\midrule
\multicolumn{10}{c}{\textbf{\textit{Prediction Horizon = 120 minutes}}}\\
\midrule

\textbf{Base} & 18.64 \scriptsize{(14.36)} & 0.56 \scriptsize{(0.77)} & 80.80 \scriptsize{(14.83)} & 94.71 \scriptsize{(2.25)} & 4.29 \scriptsize{(1.32)} & 1.00 \scriptsize{(1.03)} & 73.61 \scriptsize{(7.63)} & 12.04 \scriptsize{(4.45)} & 14.35 \scriptsize{(4.79)}\\
\midrule
\textbf{Poly} & 0.11 \scriptsize{(0.33)} & \textbf{0.00 \scriptsize{(0.00)}} & 99.89 \scriptsize{(0.33)} & \textbf{99.27 \scriptsize{(0.33)}} & \textbf{0.68 \scriptsize{(0.31)}} & \textbf{0.05 \scriptsize{(0.06)}} & \textbf{79.88 \scriptsize{(7.80)}} & \textbf{2.11 \scriptsize{(1.35)}} & 18.02 \scriptsize{(7.57)}\\
\textbf{AR} & 1.79 \scriptsize{(2.87)} & 1.21 \scriptsize{(2.05)} & 96.99 \scriptsize{(4.91)} & 85.47 \scriptsize{(8.54)} & 12.55 \scriptsize{(7.69)} & 1.97 \scriptsize{(0.96)} & 70.86 \scriptsize{(9.01)} & 14.08 \scriptsize{(5.62)} & 15.06 \scriptsize{(4.69)}\\
\textbf{ARX} & 2.46 \scriptsize{(4.07)} & 1.32 \scriptsize{(2.16)} & 96.23 \scriptsize{(6.21)} & 84.82 \scriptsize{(8.61)} & 13.06 \scriptsize{(7.75)} & 2.12 \scriptsize{(0.96)} & 70.77 \scriptsize{(8.31)} & 14.47 \scriptsize{(5.51)} & 14.75 \scriptsize{(4.44)}\\
\midrule
\textbf{SVR} & 15.23 \scriptsize{(13.46)} & 2.16 \scriptsize{(1.93)} & 82.61 \scriptsize{(14.21)} & 91.33 \scriptsize{(4.57)} & 7.67 \scriptsize{(3.86)} & 1.00 \scriptsize{(0.74)} & 75.96 \scriptsize{(6.44)} & 14.40 \scriptsize{(3.18)} & 9.64 \scriptsize{(3.55)}\\
\textbf{GP} & 3.14 \scriptsize{(4.36)} & 1.15 \scriptsize{(2.12)} & 95.71 \scriptsize{(6.31)} & 86.56 \scriptsize{(7.22)} & 11.80 \scriptsize{(6.39)} & 1.64 \scriptsize{(0.88)} & 72.49 \scriptsize{(6.75)} & 18.15 \scriptsize{(3.83)} & 9.36 \scriptsize{(3.65)}\\
\midrule
\textbf{ELM} & 17.36 \scriptsize{(13.11)} & 2.69 \scriptsize{(2.70)} & 79.95 \scriptsize{(14.18)} & 89.63 \scriptsize{(4.38)} & 9.16 \scriptsize{(3.68)} & 1.21 \scriptsize{(0.75)} & 76.49 \scriptsize{(7.35)} & 15.72 \scriptsize{(4.22)} & 7.79 \scriptsize{(3.21)}\\
\textbf{FFNN} & \textbf{33.49 \scriptsize{(16.97)}} & 2.37 \scriptsize{(2.19)} & \textbf{64.14 \scriptsize{(18.14)}} & 88.61 \scriptsize{(2.36)} & 10.50 \scriptsize{(1.94)} & 0.89 \scriptsize{(0.45)} & 75.69 \scriptsize{(3.65)} & 19.58 \scriptsize{(1.95)} & \textbf{4.73 \scriptsize{(2.05)}}\\
\textbf{LSTM} & 11.12 \scriptsize{(11.32)} & 2.89 \scriptsize{(2.44)} & 85.99 \scriptsize{(12.99)} & 89.86 \scriptsize{(5.12)} & 9.00 \scriptsize{(4.48)} & 1.14 \scriptsize{(0.69)} & 77.42 \scriptsize{(4.72)} & 14.11 \scriptsize{(2.26)} & 8.47 \scriptsize{(3.23)}\\


\bottomrule

\end{tabularx}


\begin{flushright}
AP: Accurate Prediction; BE: Benign Error; EP: Erroneous Prediction
\end{flushright}


\end{table*}

